Finite Feynman Integrals

We describe an algorithm to organize Feynman integrals in terms of their infrared properties. Our approach builds upon the theory of Landau singularities, which we use to classify all configurations of loop momenta that can give rise to infrared divergences. We then construct bases of numerators for arbitrary Feynman integrals, which cancel all singularities and render the integrals finite. Through the same analysis, one can also classify so-called evanescent and evanescently finite Feynman integrals. These are integrals whose vanishing or finiteness relies on properties of dimensional regularization. To illustrate the use of these integrals, we display how to obtain a simpler form for the leading-color two-loop four-gluon scattering amplitude through the choice of a suitable basis of finite integrals. In particular, when all gluon helicities are equal, we show that with our basis the most complicated double-box integrals do not contribute to the finite remainder of the scattering amplitude.

==> Sections/Extra.tex <==
Let us start with some well known definitions which will be useful in the following. The generalized Kronecker symbol with $R$ indices in $D$ space-time dimensions
can be defined as
\begin{equation} 
\delta^{\mu_1...\mu_R}_{\nu_1...\nu_R} \equiv 
\begin{vmatrix}
\delta^{\mu_1}_{ \nu_1} && \delta^{\mu_1}_{ \nu_2} && ... && \delta^{\mu_1}_{ \nu_R} \\[3pt]
\delta^{\mu_2}_{ \nu_1} && \delta^{\mu_2}_{ \nu_2} && ... && \delta^{\mu_2}_{ \nu_R} \\[3pt]
 &&  && ... &&  \:\\[3pt]
\delta^{\mu_R}_{ \nu_1} && \delta^{\mu_R}_{ \nu_2} && ... && \delta^{\mu_R}_{ \nu_R}  \:
\end{vmatrix} \,.\label{eq:genkron}
\end{equation} 
Whenever $D=R$, one has the obvious identity
%
\begin{equation}
    \delta^{\mu_1...\mu_R}_{\nu_1...\nu_R} 
    = \varepsilon^{\mu_1...\mu_R} \varepsilon_{\nu_1...\nu_R} \, ,
\end{equation}
%
where $\varepsilon^{\mu_1...\mu_R}$ is the Levi-Civita tensor in $R$ dimensions.
With this, we can easily define the generalized 
Gram determinant of two sets of $R$ vectors
in $D$ dimensions as
%
\begin{equation}
   \Gram{p_1  & \dots & p_R}{q_1 & \dots & q_R} = \delta^{\mu_1...\mu_R}_{\nu_1...\nu_R} p_{1 \mu_1} ... p_{R \mu_R} q_{1}^{ \nu_1} ... q_{R}^{ \nu_R} 
   =
   \delta^{p_1...p_R}_{q_1...q_R}
   \label{eq:gram_def}
\end{equation}
%
where we also introduce the standard abbreviated notation
$$\delta^{\mu_1...\mu_j...\mu_R}_{\nu_1...\nu_i...\nu_R} p_{j \mu_j} q_{i}^{ \nu_i} = \delta^{\mu_1...p_j...\mu_R}_{\nu_1...q_i...\nu_R}\,.$$
With these definitions the standard Gram determinant of $R$ vectors $p_1$, ..., $p_R$ can be expressed as
\begin{equation}
   \GramO{p_1  & \dots & p_R}
   \equiv \Gram{p_1  & \dots & p_R}{p_1 & \dots & p_R}\,. 
   \label{eq:gram}
\end{equation}

Finally, given a set of $R < D$ vectors $p_i$, 
we define the well known Van Neerven--Vermaseren basis as
\begin{equation}
  v_i^{\mu} \equiv \frac{\delta^{p_1...\mu_i...p_R}_{p_1...p_i...p_R}}{\GramO{p_1 & \dots & p_R}} \label{eq:vannver}
\end{equation}
which has the important property
\begin{equation}
    v_i \cdot p_j = \delta_{ij} \quad \mbox{for}\; j \leq R\,.
\end{equation}
In addition we note that any momentum $w^\mu$ can be decomposed on the van Neerven--Vermaseren basis as
%
\begin{equation}
    w^{\mu} = \sum_{j=1}^n (v_j \cdot w) \: k_j^\mu + \hat{w}^{\mu} \, .
\end{equation}
%
We stress here that all these definitions can be easily continued to $D$ \emph{continuous space-time dimensions}, whenever necessary.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As we have previously argued, a possile set of natural object to do so are Gram determinants together with propagator denominators.

Let us start with generators of degree two in the loop-momenta. 
As seen above, the collinear singularities of concern in $\ell_1$ arise when $\ell_1\parallel k_1$; $\ell_1-k_1\parallel k_1$; $\ell_1-k_{12}\parallel k_2$.  Similarly, the collinear singularities of concern in $\ell_2$ arise when $\ell_2\parallel k_4$; $\ell_2-k_4\parallel k_4$; and $\ell_2-k_{34}\parallel k_3$.  
The simplest Gram determinant that vanishes in all these regions is,
%
\begin{equation}
    \Gram{\ell_1&1&2}{\ell_2&3&4}\,,
\label{Degree2Gram1}    
\end{equation}
%
which also vanishes in the soft regions $\ell_1-k_1\sim 0$
and $\ell_2-k_4\sim 0$.  We can obtain a second degree-2 numerator with the same properties by splitting the vanishing factors into separate Gram determinants,
%
\begin{equation}
    \Gram{\ell_1&1&2}{1&2&4} \Gram{\ell_2&3&4}{1&2&4}\,.
\label{Degree2Gram2}
\end{equation}
%
As it turns out, these two polynomials suffice to generate the
degree-two finite numerators.  We can show sufficiency and
completeness thorugh the following procedure.  First, compute the Gr\"obner
basis $\GB1$ of the numerators of degree two obtained in the previous section,  using as variables
%
\begin{equation}
    \{\ell_i^2,\ell_1\cdot\ell_2,\ell_i\! \cdot \!k_j\}\,,
\end{equation}
%
(we use degree reverse lexicographic monomial ordering, but any
ordering will do).
Then show that the expressions~(\ref{Degree2Gram1},\ref{Degree2Gram2})
have no remainder when reduced over it.  Then compute the Gr\"obner
basis $\GB2$ of the two candidate Grams, and show that the
previously obtained numerators have no remainder when reduced over
$\GB2$. 

%Alternatively, we can compute the reduced Gr\"obner bases for both sets of expressions, and show that they are the same.

Note there are other Gram determinants that we could write down, for example
%
\begin{equation}
    \Gram{\ell_1&1&2&4}{\ell_2&1&2&4}\,,
\end{equation}
%
but this polynomial is expressible as a linear combination of
those in \cref{Degree2Gram1,Degree2Gram2}.

At higher degree in the loop momentum, starting from degree 3, we have another way of ensuring
finiteness: eliminating the propagators between the pairs of massless
legs.  For example, we can use the propagator denominator $(\ell_1-k_1)^2$
to eliminate the propagator between $k_1$ and $k_2$.  This will also
eliminate the soft singularity due to $\ell_1$, and the collinear 
singularities associated with $\ell_1$.  Increasing the polynomial
degree also allows for a larger number of Gram factors, for example
repeating some of the lines in \cref{Degree2Gram2}. Iterating this process rank by rank allows 
we obtain a full set of generators.
In \cref{tab:PlanarDoubleBoxGrams} we present a possible choice for the generators of the finite and $\Ord(\eps)$ ideals in the Gram determinat basis; they correspond to the numbers in rows 2 and 5 of \cref{tab:dbox_count}.
%
%
%
\begin{table}[hbt]
  \centering
  \begin{tabular}{lll}
    \toprule
    rank-2 finite
    &
    \( \Gram{\ell_1 & 1 & 2}{1 & 2 & 4}\,
       \Gram{\ell_2 & 3 & 4}{1 & 2 & 4}
    \)\,,
    &
    \( \Gram{\ell_1 & 1 & 2}{\ell_2 & 3 & 4}
    \)
    \\
    \addlinespace
    rank-3 finite
    &
    \( \GramO{\ell_1 & 1 & 2}
       \Gram{\ell_2 & 3 & 4}{1 & 2 & 4}
    \)\,,
    &
    \( \GramO{\ell_2 & 3 & 4}\,
       \Gram{\ell_1 & 1 & 2}{1 & 2 & 4}
    \)\,,
    \\
    \addlinespace
    &
    \(
    \left( \ell_1-k_1 \right)^2\,
           \Gram{\ell_2 & 3 & 4}{1 & 2 & 4}
    \)\,,
    &
    \(
    \left( \ell_2-k_4 \right)^2\,
        \Gram{\ell_1 & 1 & 2}{1 & 2 & 4}
    \)
    \\
    \addlinespace
    rank-4 finite
    &
    \(
    \left( \ell_1-k_1 \right)^2\,
           \GramO{\ell_2 & 3 & 4}
    \)\,,
    &
    \(
    \left( \ell_2-k_4 \right)^2\,
           \GramO{\ell_1 & 1 & 2}
    \)\,,
    \\
    \addlinespace
    &
    \(
    \left( \ell_1-k_1 \right)^2\,
    \left( \ell_2-k_4 \right)^2
    \)
    &
    \\
    \addlinespace
    rank-4 \(\mathcal{O}(\epsilon)\)
    &
    \( \GramO{\ell_1 & \ell_2 & 1 & 2 & 4}
    \)
    &
    \\
    \bottomrule
  \end{tabular}
    \caption{Double box: generators of the finite and $\Ord(\eps)$ ideals in the Gram determinat basis.}
  \label{tab:PlanarDoubleBoxGrams}
\end{table}
%
%
%
We check that the proposed generators do \textit{not\/} reduce to zero under
division by the Gr\"obner basis of degree-two numerators, which ensures
their independence. 

Notice that numerators leading to evanescent integrals can also be put into
a simple form using Gram determinants.  Here, the key additional
observation is that one of the Gram determinants should have five
or more arguments on each line, so that it naturally vanishes in
four dimensions.  The procedure of \cref{sec:IR}, leading to
a set of finite numerators, does not distinguish between those of
$\Ord(\eps^0)$ and those of $\Ord(\eps)$.  It is convenient to
eliminate the generators of the evanescent integrals from the list of
finite generators, and the results displayed in our tables follow
this separation.


\subsection{Three-loop Ladder}

The analysis of the three-loop ladder integral is quite straightforward,
and follows the same approach as for the planar double box.  Indeed,
at all ranks, some of the generators of the double box can be
taken as generators here, with the simple replacement 
$\ell_2\rightarrow\ell_3$ corresponding to the labeling of the
right-hand `outer' loop.  At rank 2, there are no additional
generators.  At rank 3, we have two additional generators involving all
three loop momentum.  This pattern repeats at rank 4, again with
two additional generators.  There are no new finite generators 
beyond rank 4.  As in the planar double box, some of the generators
correspond to daughter integrals, rather than the three-loop ladder
topology.

For the evanescent generators, we can once again
take the lone generator for the planar double
as a generator here with the replacement $\ell_2\rightarrow\ell_3$.
There are three additional generators at rank 4; and we have new generators
at ranks 5 and~6 as well.  The rank-6 generators correspond to daughter
`triangle-double boxes'.

\begin{itemize}
\item Very straightforward, same code
\item Discuss the table
\end{itemize}


\begin{table}[htb!]
  \centering
  \caption{Three-loop ladder}
  \begin{tabular}{lccccccc}
    \toprule
    rank & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\
    \midrule
    \addlinespace
    \# finite integrals & 0 & 2 & 26 & 184 & 850 & 2807 & 6044 \\
    \addlinespace
    \# finite generators & 0 & 2 & 6 & 9 & 0 & 0 & 0 \\
    \addlinespace
    \# \(\mathcal{O}(\epsilon)\) integrals & 0 & 0 & 0 & 4 & 42 & 229 & 678 \\
    \addlinespace
    \# \(\mathcal{O}(\epsilon)\) generators & 0 & 0 & 0 & 4 & 2 & 2 & 0 \\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}[htb!]
  \centering
  \begin{tabular}{lll}
    \toprule
    rank-2 finite
    &
    \( \Gram{\ell_1 & 1 & 2}{1 & 2 & 4}\,
       \Gram{\ell_3 & 3 & 4}{1 & 2 & 4}
    \)\,,
    &
    \( \Gram{\ell_1 & 1 & 2}{\ell_3 & 3 & 4}
    \)
    \\
    \addlinespace
    rank-3 finite
    &
    \( \GramO{\ell_3 & 3 & 4}\,
       \Gram{\ell_1 & 1 & 2}{1 & 2 & 4}
    \)\,,
    &
    \( \GramO{\ell_1 & 1 & 2}\,
       \Gram{\ell_3 & 3 & 4}{1 & 2 & 4}
    \)\,,
    \\
    \addlinespace
    &
    \( \Gram{\ell_3 & 3 & 4}{\ell_2 & 3 & 4}\,
       \Gram{\ell_1 & 1 & 2}{1 & 2 & 4}
    \)\,,
    &
    \( \Gram{\ell_1 & 1 & 2}{\ell_2 & 1 & 2}\,
       \Gram{\ell_3 & 3 & 4}{1 & 2 & 4}
    \)\,,
    \\
    \addlinespace
    &
    \(
    \left( \ell_3+k_4 \right)^2\,
        \Gram{\ell_1 & 1 & 2}{1 & 2 & 4}
    \)\,,
    &
    \(
    \left( \ell_1-k_1 \right)^2\,
       \Gram{\ell_3 & 3 & 4}{1 & 2 & 4}
    \)
    \\
    \addlinespace
    rank-4 finite
    &
    \(
    \left( \ell_3+k_4 \right)^2\,
        \Gram{\ell_1 & 1 & 2}{\ell_2 & 1 & 2}
    \)\,,
    &
    \(
    \left( \ell_1-k_1 \right)^2\,
        \Gram{\ell_3 & 3 & 4}{\ell_2 & 3 & 4}
    \)\,,
    \\
    \addlinespace
    &
    \(
    \left( \ell_3+k_4 \right)^2\,
        \GramO{\ell_1 & 1 & 2}
    \)\,,
    &
    \(
    \left( \ell_1-k_1 \right)^2\,
        \GramO{\ell_3 & 3 & 4}
    \)\,,
    \\
    \addlinespace[2ex]
    &
    \(
    \left( \ell_1-k_1 \right)^2\,
    \left( \ell_3+k_4 \right)^2
    \)
    &
    \\
    \addlinespace
    rank-4 \(\mathcal{O}(\epsilon)\)
    &
    \( \GramO{\ell_1 & \ell_3 & 1 & 2 & 4}
    \)\,,
    &
    \( \Gram{\ell_1 & \ell_2 & 1 & 2 & 4}{\ell_2 & \ell_3 & 1 & 2 & 4}
    \)\,,
    \\
    \addlinespace
    &
    \( \Gram{\ell_1 & \ell_2 & 1 & 2 & 4}{\ell_1 & \ell_3 & 1 & 2 & 4}
    \)\,,
    &
    \( \Gram{\ell_1 & \ell_3 & 1 & 2 & 4}{\ell_2 & \ell_3 & 1 & 2 & 4}
    \)
    \\
    \addlinespace
    rank-5 \(\mathcal{O}(\epsilon)\)
    &
    \( \Gram{\ell_1 & \ell_2 & 1 & 2 & 4}{\ell_1 & \ell_2 & \ell_3 & 3 & 4}
    \)\,,
    &
    \( \Gram{\ell_2 & \ell_3 & 1 & 2 & 4}{\ell_1 & \ell_2 & \ell_3 & 1 & 2}
    \)
    \\
    \addlinespace
    rank-6 \(\mathcal{O}(\epsilon)\)
    &
    \(
    \left( \ell_3+k_4 \right)^2\,
       \GramO{\ell_1 & \ell_2 & 1 & 2 & 4}
    \)\,,
    &
    \(
    \left( \ell_1-k_1 \right)^2\,
        \GramO{\ell_2 & \ell_3 & 1 & 2 & 4}
    \)
    \\
    \bottomrule
  \end{tabular}
    \caption{Three-loop ladder: Gram generators \GG{Need to check this again, but I think the rank 5 and rank 6 generators don't exist, see \cref{eq:ladder_conjecture}}}
\end{table}









\subsection{Canonical Forms for Numerators}
\label{sec:canonical_numerators}

\GG{this subsection still to be finished}
The procedure outlined in previous sections allows us to give a
complete account of integrands leading to locally finite integrals. The collections of these integrands form ideals, with a limit on the degree of polynomials imposed by UV-finiteness. \GG{maybe we want to describe them as \textit{graded ideals}?}\LT{graded in what, in UV powercouting? a grading must be respected by some operation in the space considered usually?}\GG{The ideal is graded with respect to the scaling of loop momenta. Each sub-integration induces a grading of ideal and we want to take the itersection of the lowest modules.. I'm not sure about the vocabulary here.}
Describing locally finite numerators in terms of the monomials in \cref{eq:monomials} is not particularly illuminating, however.
As an alternative, we can use computational algebraic geometry, in particular Gr\"obner bases,
to obtain a compact set of generators; but the ones that emerge
from this computation are not very natural either.

Instead, we can exploit the fact that all singularities that we encounter are either soft or collinear and identify a set of objects which naturally vanish on such configurations of the loop momenta. Natural objects to use to make this interpretation manifest, are then Gram determinants defined in~\cref{eq:gram_def} and~\cref{eq:gram}.
For the sake of compactness, here and below, we indentify external momenta in Gram determinant arguments with their index, $e.g.$ 
$$G(k_1 \; k_2 \;\dots) \equiv G(1\; 2\;\dots)\,.$$ 
%
% \begin{equation} \label{eq:gram_def}
%     \Gram{p_1&p_2& \dots &p_n}{q_1&q_2& \dots &q_n} = \det_{i,j}(2p_i\cdot q_j) \,, \quad  \GramO{p_1&p_2& \dots &p_n} = \Gram{p_1&p_2& \dots &p_n}{p_1&p_2& \dots &p_n} \,.
% \end{equation}
%
The generalised Gram determinants $\Gram{p_1&p_2& \dots &p_n}{q_1&q_2& \dots &q_n}$, clearly vanish nontrivially when either the $p_i$'s or the $q_i$'s are linearly dependent. In particular they automatically vanish in all collinear limits. Since collinear singularities are all logarithmic\footnote{Recall that we are considering integrals which are a superset of those arising in Yang--Mills theory, and so the logarithmic nature of soft singularities is not guaranteed.} \cite{} \GG{citation/explanation?} any degree of vanishing of the numerator in corresponding momentum configurations suffices to render its contribution finite. \GG{Do we have something to say about non logarithmic soft singularities here?}

An additional benefit is that Gram determinants with five or more momentum arguments on each line will necessarily vanish in four dimensions. 

This prompts us to find a generating set built out of Gram determinants. As we shall see, we can indeed find a set built out of Gram determinants and propagator denominators. Here we do not set forth a mechanical procedure for finding the generators, but leave this subject to future investigation. Instead we provide various examples in \cref{sec:results}.




\begin{table}[tbh!]
  \centering
  \caption{Nonplanar double box: Gram generators \draftnote{What is the reason for $i$ and $i+1$? --DAK}}
  \begin{tabular}{ll}
    \toprule
    rank-3 finite
    &
    \( \Gram{\ell_1 & 1 & 2}{1 & 2 & 4}\,
       \Gram{\ell_2 & 4}{i & i+1}\,
       \Gram{\ell_1 + \ell_2 & 3}{i & i+1}
    \)\,,\quad
%    \\
%    \addlinespace
%    &
    \( \Gram{\ell_2 & 4}{\ell_1 + \ell_2 & 3}\,
       \Gram{\ell_1 & 1 & 2}{1 & 2 & 4}
    \)
    \\
    \addlinespace
    &
    \( \Gram{\ell_2 & 4}{1 & 2}\,
       \Gram{\ell_1 & 1 & 2}{\ell_1 + \ell_2 & 3 & 1}
    \)\,,\quad
%    \\
%    \addlinespace
%    &
    \( \Gram{\ell_2 & 4}{2 & 3}\,
       \Gram{\ell_1 & 1 & 2}{\ell_1 + \ell_2 & 3 & 1}
    \)\,,
    \\
    \addlinespace
    &
    \( \Gram{\ell_1 + \ell_2 & 3}{1 & 2}\,
       \Gram{\ell_1 & 1 & 2}{\ell_2 & 4 & 1}
    \)\,,\quad
%    \\
%    \addlinespace
%    &
    \( \Gram{\ell_1 + \ell_2 & 3}{2 & 3}\,
       \Gram{\ell_1 & 1 & 2}{\ell_2 & 4 & 1}
    \)
    \\
    \addlinespace
    rank-4 finite
    &
    \(
    \left( \ell_1-k_1 \right)^2\,
           \Gram{\ell_2 & 4}{i & {i+1}}\,
           \Gram{\ell_1 + \ell_2 & 3}{i & {i+1}}
    \)\,,\quad
%    \\
%    \addlinespace
%    &
    \(
    \left( \ell_1-k_1 \right)^2\,
           \Gram{\ell_2 & 4}{\ell_1 + \ell_2 & 3}
    \)\,,
    \\
    \addlinespace
    &
    \( \GramO{\ell_1 & 1 & 2}\,
       \Gram{\ell_2 & 4}{\ell_1 + \ell_2 & 3}
    \)\,,\quad
%    \\
%    \addlinespace
%    &
    \( \Gram{\ell_1 & 1 & 2}{\ell_2 & 1 & 2}\,
       \Gram{\ell_2 & 4}{\ell_1 + \ell_2 & 3}
    \)
    \\
    \addlinespace
    rank-4 \(\mathcal{O}(\epsilon)\)
    &
    \( \GramO{\ell_1 & \ell_2 & 1 & 2 & 4}
    \)
    \\
    \bottomrule
  \end{tabular}
\end{table}









\subsection{Three-loop ladder}

\pavel{TODO}

We give two examples of IR--IR evanescently finite numerators for the 
three-loop ladder:
\begin{subequations}
  \begin{align}
    \mathrm{Num}_1 &= \mathrm{G}
    \begin{pmatrix}
      \ell_2 & \ell_3 & 1 & 2 & 4 \\
      \ell_1 & \ell_2 & \ell_3 & 1 & 4
    \end{pmatrix}
    , \\
    \mathrm{Num}_2 &= \ell_1^2 \, \mathrm{G}
    \begin{pmatrix}
      \ell_2 & \ell_3 & 1 & 2 & 4
    \end{pmatrix}
    ,
  \end{align}
\end{subequations}
which cancel all IR divergences except for a collinear one
when \(\ell_1 = k_1 + x k_2\).
(In fact, one can check that \(s_{12} \mathrm{Num}_1 + \mathrm{Num}_2\) 
cancels this IR divergence, so these two numerators are linearly dependent 
\enquote{modulo} the locally finite truncated ideal.)





\section{evanescently finite for double box}
% TODO Pavel: continue here
\pavel{Improve text}
\pavel{Mention that these are UV--IR cancellations}

We have checked that all possible logarithmically UV-divergent integrals with 
evanescent numerators (proportional to 
\(\mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix} \)) are
finite.

More precisely:
\begin{enumerate}
\item \(\left( \ell_1 \cdot \ell_2 \right) \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\) gives a finite integral;
\item Likewise for \(\left( \ell_1 \cdot k_i \right) \left( \ell_2 \cdot k_j \right) \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\) with \(i \neq j\);
\item \(\left( \ell_1 \cdot k_i \right) \left( \ell_2 \cdot k_i \right) \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\) 
gives an integral of \(\mathcal{O}(\epsilon)\).
\end{enumerate}

We have also checked a few integrals with a power-like UV divergence caused by an additional logarithmic \(\ell_1\) subdivergence.
Naively one would expect them to be of \(\mathcal{O}(1/\epsilon)\), 
but some of them are actually \(\mathcal{O}(\epsilon)\):
\begin{enumerate}
\item \(\left( \ell_1 \cdot k_i \right) \left( \ell_1 \cdot k_j \right) \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\) with \(i \neq j\) 
indeed gives an integral of \(\mathcal{O}(1/\epsilon)\);
\item \(\left( \ell_1 \cdot k_i \right)^2 \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\), in contrast, gives an integral 
of \(\mathcal{O}(\epsilon)\).
\end{enumerate}



\subsubsection{Evanescently Finite Integrals for npl double box}

\pavel{Improve text}
\pavel{Mention that these are UV--IR cancellations}

We have checked that all possible logarithmically UV-divergent integrals with 
evanescent numerators (proportional to 
\(\mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix} \)) are
finite:
\begin{enumerate}
\item \(\left( \ell_1 \cdot \ell_2 \right) \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\) gives a finite integral;
\item Likewise for \(\left( \ell_1 \cdot k_i \right) \left( \ell_2 \cdot k_j \right) \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\) with \(i \neq j\);
\item \(\left( \ell_1 \cdot k_i \right) \left( \ell_1 \cdot k_j \right) \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\) with \(i \neq j\) also gives a finite integral;
\item \(\left( \ell_1 \cdot k_i \right) \left( \ell_2 \cdot k_i \right) \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\) gives
an integral of \(\mathcal{O}(\epsilon)\);
\item Likewise for \(\left( \ell_1 \cdot k_i \right)^2 \mathrm{G} \begin{pmatrix} \ell_1 & \ell_2 & 1 & 2 & 4 \end{pmatrix}\).
\end{enumerate}


